Shallow Neural Hawkes: Non-parametric kernel estimation for Hawkes processes

Multi-dimensional Hawkes process (MHP) is a class of self and mutually exciting point processes that find wide range of applications -- from prediction of earthquakes to modelling of order books in high frequency trading. This paper makes two major contributions, we first find an unbiased estimator for the log-likelihood estimator of the Hawkes process to enable efficient use of the stochastic gradient descent method for maximum likelihood estimation. The second contribution is, we propose a specific single hidden layered neural network for the non-parametric estimation of the underlying kernels of the MHP. We evaluate the proposed model on both synthetic and real datasets, and find the method has comparable or better performance than existing estimation methods. The use of shallow neural network ensures that we do not compromise on the interpretability of the Hawkes model, while at the same time have the flexibility to estimate any non-standard Hawkes excitation kernel.

==> Neural Hawkes paper for arxiv/Experiments_and_results.tex <==
\subsection{Synthetic Data}
In this section we demonstrate the performance of the Shallow Neural Hawkes model by fitting various forms of kernels and by weighing it against state-of-the-art non-parametric models, including EM method given in \citet{lewis2011nonparametric} and Wiener-Hopf (WH) model described in \citet{bacry2014second}. All simulations are performed using the thinning algorithm described in \citet{ogata1981lewis}. We also use large set of tools from the tick library, \citet{bacry2017tick}, that facilitates efficient parametric and non-parametric estimations. Here we examine the univariate case of Hawkes process, followed by the bivariate case.

\subsubsection{Univariate Case} \label{univariate}
First, we simulate univariate Hawkes process for widely used forms of kernels, namely 
\begin{equation}	
\text{Exponential kernel: } ~~~\phi(t) = \alpha e^{-\beta t}
\end{equation}  
\begin{equation}
\text{Power Law kernel: }~~~ \phi(t) = \alpha (\delta+t)^{-\beta}
\end{equation}  

Next, we verify the performance of the Shallow Neural Hawkes model on a rectangular kernel given by,
\begin{equation}
\phi(t) = \begin{cases}
              \alpha \beta, & \text{if}\ \delta < t < \delta + \dfrac{1}{\beta} \\
              0, & \text{otherwise}
              \end{cases}
\end{equation}  

\textbf{Experiment setup :} 
For the exponential kernel simulation, we use parameters $[ \alpha, \beta, \mu] = [1,4,0.05]$, for a period of $[0,60000)$ and we get $N_T = 3972$ events. Similarly, for the simulation of power law kernel, we use parameters $[ \alpha, \beta, \delta, \mu] = [1,4,1,0.05]$, for a period of $[0,60000]$ and get $N_T = 4442$ events. We use  $100$ neurons for each kernel and the initial weights are drawn from uniform distribution in the range of $[0,0.5].$ In all our initializations we find that positive weights for the inner layer and negative weights for the outer layer helps in faster convergence of the algorithm. This initial setting is common to all experiments in this paper. We use ADAM optimizer \citet{kingma2014adam}, set the batch size to 50 and employ varied learning rates for the parameters of the inner and the outer layer. We find by default using a learning rate of  $10^{-2}$ for the outer layer and $10^{-5}$ for the inner layer, and $10^{-3}$ for $\mu$ gives reasonably good results. We train the network up to 30 epochs. 

The rectangular kernels are simulated using parameters $[ \alpha, \beta, \delta, \mu] = [0.7,0.4,1,0.05]$, for a period of $[0,60000]$ and we get $N_T = 10196$ events. Implementation details for the SNH model is similar to the above setting. The learning rate for outer layer is $10^{-2}$, for inner layer is $5 \times 10^{-4}$ and for $\mu$ is $10^{-3}$. The model is trained for 30 epochs.  When the excitation kernels are smooth we find using smaller learning rates for the inner layer can significantly improve the convergence, although for kernels with inflection points (like the rectangular kernel) a relatively higher learning rate for the inner layer helps. For all the cases we find that using a higher learning rate for the output layer in comparison to the learning rate for the input layer helps in faster convergence. 

The learned kernels from the Shallow Neural Hawkes model are then compared to kernels determined by the parametric sum of exponential kernels method, non-parametric EM and WH model, as shown in Figure \ref{Synthetic_data}. These models are implemented using the tools provided in tick library \citet{bacry2017tick}.For the non-parametric EM estimation, we choose the kernel support as $5$ and kernel size of $20$. For the WH method, we set the number of quadratures as $50$ and use linear sampling for exponential kernels. However, the linear sampling method performs poorly in the case of power law kernel and rectangular kernel, hence we use the semi-log sampling approach with maximum kernel support of $1000$ and maximum lag as $100$. The next section provides a detailed description of the observations.

\textbf{Experiment results :} 
First, we compare the performance of non-parametric models based on the kernel estimation approach. The EM model is a histogram based estimator with discrete function kernel, whose performance critically depends on the choice of bins. WH model also has a strong dependancy on the choice of grid in the kernel estimation process \citet{morzywolek2015non} . On the contrary, the Shallow Neural Hawkes model provides a continuous function kernel and does not rely on the range of kernels, a vital advantage of the model. 

From a visual assessment of the kernel estimation plot in \ref{Synthetic_data} , it is evident that the Shallow Neural Hawkes model outperforms the former models in the exponential and power law kernel estimation and exhibits a finer performance in the case of the rectangle kernel. Next on the evaluation metrics, we plot the L1 error, defined as $|\phi - \phi_{\text{est}}|$, between the true and estimated kernels of all the models in comparison, refer Figure\ref{Synthetic_data}. We observe that the error is consistently significantly lower in the case of Shallow Neural Hawkes. Figure\ref{Synthetic_data} also shows the convergence of the system, the negative log-likelihood estimated in the Shallow Neural Hawkes model reaches the true negative log-likelihood precisely within 10 epochs. We have verified that speed of convergence is higher for larger sample periods. 

\begin{figure}
  \centering
  \begin{subfigure}[b]{0.3\linewidth}
    \includegraphics[width=\linewidth]{Images/1D_Exp_kernel.png}
    \caption{}
  \end{subfigure}
  \begin{subfigure}[b]{0.3\linewidth}
    \includegraphics[width=\linewidth]{Images/1D_Exp_error.png}
    \caption{}
  \end{subfigure}
  \begin{subfigure}[b]{0.3\linewidth}
    \includegraphics[width=\linewidth]{Images/1D_Exp_convergence.png}
    \caption{}
  \end{subfigure}
  \begin{subfigure}[b]{0.3\linewidth}
    \includegraphics[width=\linewidth]{Images/1D_Power_kernel.png}
    \caption{}
  \end{subfigure}
  \begin{subfigure}[b]{0.3\linewidth}
    \includegraphics[width=\linewidth]{Images/1D_Power_error.png}
    \caption{}
  \end{subfigure}
  \begin{subfigure}[b]{0.3\linewidth}
    \includegraphics[width=\linewidth]{Images/1D_Power_convergence.png}
    \caption{}
  \end{subfigure}
  \begin{subfigure}[b]{0.3\linewidth}
    \includegraphics[width=\linewidth]{Images/1D_Rec_kernel.png}
    \caption{}
  \end{subfigure}
  \begin{subfigure}[b]{0.3\linewidth}
    \includegraphics[width=\linewidth]{Images/1D_Rec_error.png}
    \caption{}
  \end{subfigure}
  \begin{subfigure}[b]{0.3\linewidth}
    \includegraphics[width=\linewidth]{Images/1D_Rec_convergence.png}
    \caption{}
  \end{subfigure}
  \caption{\footnotesize Synthetic data experiment results for univariate Hawkes processes \\ (a) The estimated Exponential kernel  (b) The estimated error for Exponential kernel  (c) The convergence plot of Negative Log-likelihood for Exponential kernel estimation in SNH model  (d) The estimated Power Law kernel  (e) The estimated error for Power Law kernel  (f) The convergence plot of Negative Log-likelihood for Power Law kernel estimation in SNH model  (g) The estimated rectangular kernel  (h) The estimated error for rectangular kernel  (i) The convergence plot of Negative Log-likelihood for rectangular kernel estimation in SNH model}
  \label{Synthetic_data}
\end{figure}


\subsubsection{Bivariate Case}
We simulate bivariate Hawkes processes for the exponential and power-law kernels using tick library, the complete experimental setup and results are discussed in the Appendix \ref{B2}. In this section, we define some random kernels to test the performance of the Shallow Neural Hawkes model, this helps us understand the versatility of our model.

\textbf{Experiment setup :} The random kernels are simulated using the TimeFunction class from tick library, it uses several types of interpolation to determine the function value between two points on $[0,\infty)$ \citet{bacry2017tick}. The kernel function $\phi_{(0,0)}(t)$ is defined using $x = [0, 1, 1.5, 2., 3.5],  y = [0, 0.2, 0, 0.1, 0.]$ and the y-values are extended to the right. Next, we have $\phi_{(0,1)}(t) = \dfrac{sin(t)}{4} ~~\text{for} ~0 < t  < T$. We then generate a zero kernel $\phi_{(1,0)}(t)$ = 0. Finally, we simulate a random form kernel for $\phi_{(1,1)}(t)$ using $x = [0., .7, 2.5, 3., 4.]$ and $y =  [.3, .03, .03, .2, 0.]$. The baseline values are set at $\mu = [0.05, 0.05]$. To recover the random kernels using SNH model, we use the same network setting as above with the learning rate for the inner layer set to $5 \times 10^{-4}$. We train the network for 100 epochs.

\textbf{Experiment results :} Here we discuss the performance of the SNH model on random kernels, as shown in Figure \ref{Synthetic_data_2}. We see that the kernel setting in $\phi_{0,0}(t)$ is highly disadvantageous to the SNH model. However, the EM model exhibits an impressive performance in fitting $\phi_{0,0}(t)$, while the WH struggles to capture this function. In the case of kernels  $\phi_{0,1}(t) , \phi_{1,0}(t), \phi_{1,1}(t)$, the SNH model achieve better results when compared to other models and this serves as proof that our can be applicable to a diverse class of non-parametric Hawkes processes.

Finally, we have verified that the SNH model accurately recovers the baseline values in both, univariate and bivariate case of Hawkes processes.

\begin{figure}
  \centering
  \begin{subfigure}[b]{0.4\linewidth}
    \includegraphics[width=\linewidth]{Images/2D_random_kernels.png}
    \caption{}
  \end{subfigure}
  \begin{subfigure}[b]{0.4\linewidth}
    \includegraphics[width=\linewidth]{Images/2D_random_error.png}
    \caption{}
  \end{subfigure}
  \caption{\footnotesize Synthetic data experiment results for bivariate Hawkes processes with random kernels \\ (a) The estimated random kernels  (b) The estimated error for random kernels}
  \label{Synthetic_data_2}
\end{figure}

\subsection{Real Data}
A growing literature is dedicated to study the application of point processes to high frequency financial data. In particular, due to the correlated and clustered nature of trading activity, Hawkes processes are used to model trade arrival dynamics. A continuous time bivariate Hawkes process was used for modelling the arrival times of market sell and buy orders in \citet{bowsher2007modelling}. Recently, a bivariate Hawkes process was proposed in \citet{bacry2013modelling} to model the variations of asset prices and study the signature plot and the Epps effect. In this paper, we investigate the performance of the Shallow Neural Hawkes model on arrival data for buy and sell bitcoin market orders on the Binance exchange.

\textbf{Experiment setup :} We use the bitcoin data, traded in the Binance cryptocurrency exchange. The full dataset consists of 120000 intraday market orders, as recorded on 08 May 2020 covering the period between 6.45 PM to 10.55 PM (UTC), with corresponding volume and timestamps rounded to nearest second. The dataset was cleaned to include only unique market orders, as a particular market order might require several limit orders to full fill the demanded volume; with each recorded as a separate trade with a common market order id.

A bivariate analysis is performed jointly on the buy and sell trade data, to learn the interactions between them. For the SNH network architecture, we use the same initial settings as in the synthetic data instance. We set a learning rate of  $10^{-2}$ for the outer layer,  for the inner layer we use a learning rate of $10^{-3},$ and for $\mu$ a learning rate of $10^{-3}$. With $N_{T_{\text{sell}}} + N_{T_{\text{buy}}} = 83574$, we train the network in 30 epochs. 

To facilitate comparison with standard models, we perform non-parametric analysis on the bitcoin dataset using EM and WH models. For the EM estimation, we choose the kernel support as $6$ and kernel size of $100$. For the WH method, we set the number of quadratures as $200$.

\textbf{Experiment results :}  In Figure \ref{Real_data_3}, we plot the kernels estimated by SNH, EM and WH methods. It is evident that the two events are not mutually exciting, but exhibit self exciting behaviour. The negative log-likelihood values recorded from the SNH, EM and WH models are -40143, -33127, and -29698 respectively. The SNH model achieves competitive negative loglikelihood when compared to EM and WH models. We also perform a k-fold cross validation to compare the three models on limited samples of data, with negative log-likelihood used as an evaluation metric (see Appendix \ref{B3} for more details). The WH method exhibits consistently poor results while the performances of EM and SNH methods are comparable. 


\begin{figure}
 
  \centering
  \includegraphics[width=\linewidth]{Images/2D_binance_kernel.png}
  \caption{\footnotesize Experiment results of Bitcoin data as bivariate Hawkes processes. Estimated $\mu_1$ is 0.857, 0.463, 0.070 for SNH, EM and WH respectively. Estimated $\mu_2$ is 1.173, 0.685, 0.272 for SNH, EM and WH respectively. The negative log-likelihood values are -40143,-33127, -29698 for SNH, EM and WH respectively. }
%    Est $\mu 2$ &1.173 &0.685 &0.272 \\}
  \label{Real_data_3}
  
\end{figure}

%\begin{table}
%  \caption{Estimated $\mu$ and Negative Log-likelihood for bivariate Bitcoin Data}
%  \label{Real data-table 1}
%  \centering
%  \begin{tabular}{llll}
%    \toprule
%      & SNH & EM & WH  \\
%    \midrule
%    Est $\mu 1$ &0.857 &0.463 &0.070 \\
%    Est $\mu 2$ &1.173 &0.685 &0.272 \\
%    Neg Loglik& -40143 &-33127 & -29698\\
%    \bottomrule
%  \end{tabular}
%\end{table}
